Higher Criticism for Discriminating Word-Frequency Tables and Testing Authorship

We adapt the Higher Criticism (HC) goodness-of-fit test to measure the closeness between word-frequency tables. We apply this measure to authorship attribution challenges, where the goal is to identify the author of a document using other documents whose authorship is known. The method is simple yet performs well without handcrafting and tuning; reporting accuracy at the state of the art level in various current challenges. As an inherent side effect, the HC calculation identifies a subset of discriminating words. In practice, the identified words have low variance across documents belonging to a corpus of homogeneous authorship. We conclude that in comparing the similarity of a new document and a corpus of a single author, HC is mostly affected by words characteristic of the author and is relatively unaffected by topic structure.

==> table_result_trained.tex <==

\begin{tabular}{l|c|c|c}
    vocabulary size & $250$ & $1,000$ & $3,000$ \\
    \hline
    $\HC$ &  {\bf .83} (.067) & {\bf .88} (.063) & {\bf .91} (.039) \\
    % 9,0.8254509803921568,freq_table_HC,10.0,0.06622911776541056,250.0
% 10,0.8809019607843137,freq_table_HC,10.0,0.0629235330472595,1000.0
% 11,0.9109019607843137,freq_table_HC,10.0,0.03858424975432579,3000.0
    \hline
    SVM & .88 (.034) &  .89 (.033)  & .90 (.032) \\ \hline 
    % 18,0.8769411764705882,SVM,10.0,0.034402596398891254,250.0
% 19,0.8947843137254902,SVM,10.0,0.03335549436343498,1000.0
% 20,0.9049019607843137,SVM,10.0,0.03246919102800486,3000.0
    Naive Bayes & .76 (.048) & .84 (.049) & .89 (.064) \\ \hline
    % 12,0.7641568627450981,multinomial_NB,10.0,0.048281884083391576,250.0
% 13,0.8371372549019608,multinomial_NB,10.0,0.04924311398844248,1000.0
% 14,0.8867843137254902,multinomial_NB,10.0,0.06463407780606784,3000.0
Neural Network & .68 (.025) & .69 (.05) & .72 (.055) \\ 
% 3,0.675010902694068,NeuralNet,10.0,0.025218127713245844,250.0
% 4,0.6949367398739696,NeuralNet,10.0,0.05223649797228754,1000.0
% 5,0.7204078832603221,NeuralNet,10.0,0.055271882379772555,3000.0
\end{tabular}

==> tkz_sim_measures.tex <==
\begin{tikzpicture}
\begin{axis}[
    ybar,
    width=0.5\textwidth,
    height=0.4\textwidth,
    bar width=4pt,
    enlargelimits=0.05,
    enlarge x limits=0.2,
    legend style={at={(1,0.5)},
     anchor=west, %legend columns=-1
     legend cell align={left}
     },
    ylabel={accuracy},
    xlabel={vocabulary size},
    symbolic x coords={3000,1000,250},
    xticklabel style={align=center},
    xticklabels={\small {$250$},\small {$1,000$},\small {$3,000$}},
    xtick=data,
    ymin = 0,
    nodes near coords align={vertical},
    ]
 
    \addplot[draw=black, fill=red!70] table [x=vocab_size, y=freq_table_HC, col sep=comma] {./sim_measures_Gut_full_10cv.csv};
    
    \addplot[draw=black, fill=magenta!80!black] table [x=vocab_size, y=freq_table_LL, col sep=comma] {./sim_measures_Gut_full_10cv.csv};
    
    % \addplot[draw=black, fill=red!50!blue] table [x=vocab_size, y=freq_table_FT, col sep=comma] {./sim_measures_Gut_full_10cv.csv};

    \addplot[draw=black, fill=orange] table [x=vocab_size, y=freq_table_CR, col sep=comma] {./sim_measures_Gut_full_10cv.csv};
    
    \addplot[draw=black, fill=blue!50] table [x=vocab_size, y=freq_table_chisq, col sep=comma] {./sim_measures_Gut_full_10cv.csv};
    
    \addplot[draw=black, fill=green!60!black] table [x=vocab_size, y=freq_table_cosine, col sep=comma] {./sim_measures_Gut_full_10cv.csv};
    
\legend{\scriptsize $\HC$, \scriptsize $\PD_{0}$ ($G^2$), \scriptsize $\PD_{2/3}$ (Cressie-Reed), \scriptsize $\PD_2$ (Pearson's $\chi^2$),\scriptsize cosine similarity}
\end{axis}
\end{tikzpicture}

\caption{Accuracy in determining the authorship of 11,669 literary works among 488 writers using several statistics (interpreted as indices of similarity) and vocabulary sizes. Each $k$-size dictionary consists of the $k$ most frequent English words according to the list \citep{mostCommon}. Results were obtained using a 10-fold cross validation procedure.
\label{fig:Gutenberg_results}
    }
